How Much Progress Did I Make? An Unexplored Human Feedback Signal for Teaching Robots

Enhancing the expressiveness of human teaching is vital for both improving robots' learning from humans and the human-teaching-robot experience. In this work, we characterize and test a little-used teaching signal: \textit{progress}, designed to represent the completion percentage of a task. We conducted two online studies with 76 crowd-sourced participants and one public space study with 40 non-expert participants to validate the capability of this progress signal. We find that progress indicates whether the task is successfully performed, reflects the degree of task completion, identifies unproductive but harmless behaviors, and is likely to be more consistent across participants. Furthermore, our results show that giving progress does not require extra workload and time. An additional contribution of our work is a dataset of 40 non-expert demonstrations from the public space study through an ice cream topping-adding task, which we observe to be multi-policy and sub-optimal, with sub-optimality not only from teleoperation errors but also from exploratory actions and attempts. The dataset is available at https://github.com/TeachingwithProgress/Non-Expert\_Demonstrations.

==> epitaph_for_my_brain_cells.tex <==
Integrating human knowledge into robot learning has achieved a wide application in the real world.
Learning from Demonstration (LfD) greatly improves robot learning by reducing the exploration cost while learning new skills \cite{zhang2022lidar, pshikhachev2022self, brown2020better, chen2021learning}.  
However, most Learning from Demonstration (LfD) methods are based on the assumption that the demonstrations are optimal \cite{kalakrishnan2013learning, ho2016generative}, while getting optimal demonstrations, especially in robot manipulation tasks, is extremely hard.\cite{sasaki2020behavioral, palan2019learning, wang2021learning}. 
By admitting the suboptimality in demonstrations, prior work addressed the problem by auto-ranking demonstrations by quality\cite{ brown2019ranking, brown2020better}, assigning weights to demonstrations by calculating confidence or risks \cite{sasaki2020behavioral, wu2019imitation,chen2021learning}, or generating better reward functions or demonstrations using generative methods\cite{liu2019hindsight,hussein2021robust}.
While these methods have achieved great success, they still require demonstrations to be relatively high quality (or partially from experts), and assuming that there is only one policy or function in the demonstrations does not hold where demonstrations are from multiple demonstrators \cite{ravichandar2020recent}.   

On the other hand,
Learning from Human Feedback (LfHF) enables robots to better adapt to human preferences or correct wrong behaviors by shaping a learned policy or learning a new policy \cite{lin2020human,cui2021empathic, poole2021towards, najar2020interactively, cederborg2015policy, knox2009interactively}.
% Alternatively, some approaches seek to utilize side information from humans, such as human feedback.
Giving high-quality feedback can be much easier than giving high-quality demonstrations\cite{arzate2020survey}, and 
Human teaching signals can be complementary to human demonstrations. 
Human demonstrations contain more and relatively global information including policies and goals, but tend to be less accurate. Human feedback contains less and relatively local information such as the correctness of a robot's action, or preference over two trajectories, but is more accurate. 
consolidating human demonstrations and human feedback could significantly reduce the need for human feedback\cite{ibarz2018reward, palan2019learning}, improve the accuracy of the outcome of LfD\cite{ning2022learning, biyik2022learning, brown2019extrapolating}, and increase safety during policy optimization\cite{brown2020safe}.
However, even when combining human feedback with demonstrations, the data needs for human feedback are still high and often require humans to stay in the loop to interact with the robot for a long time \cite{biyik2022learning,ibarz2018reward, palan2019learning}. Moreover, the quality of a demonstration is only indicated by comparing it to another demonstration resulting in neglecting the fact that the selected demonstrations could be both good or bad which human feedback is capable of.     

In this work, we aim to enable learning from multiple naive users and only collect feedback for one time after they provide demonstrations.
We proposed a novel teaching signal, \textit{progress}, that provides both relative and objective insights of a demonstration and can be collected along with the demonstrations. 
We conducted a two-phase online study with 76 participants to collect progress with pre-recorded demonstrations from crowd users and showed progress can report weights of a partial trajectory, towards or away from task completion, if the task is completed at the end of a demonstration while the workload is similar to provide scalar evaluation. 
Then we conducted a public space study in a university building.
All demonstrators we recruited were random people who walked by in a lobby of a university building. 
People who were robot experts were excluded from our study. 
Participants were asked to provide demonstrations of a pouring task. After giving the demonstration, they were asked to further provide ten progress and ten scalar evaluations. 
Participants average only interacted with the robot for [XX] minutes.
We released all the demonstrations along with the progress and evaluations we collected. 
We proposed an effective Weighted Behavior Cloning method with progress.
We demonstrated that our method enables the robot to learn a better policy by using progress.

We have three major contributions:
\begin{enumerate}
    \item Novel teaching signal: \textit{prgress}.
    \item Non-expert demonstration data set. 
    \item A new Weighted Behavior Cloning method. 
\end{enumerate}
\hang{revisit the last part once the in-person study in done or once we have the BC method}





% \hang{rethinking this paper: what is the contribution? IRL seems not appropriate here.}
% \hang{The key contribution of this paper should be: progress}
% \hang{This could be under pure learning from evaluative feedback context but I think it might be better to do it with LfD}
% \hang{need a really clear line for this:

% \begin{itemize}
%     \item What is the online study for?
%     \item Why do we need an in-person study?
%     \item What we are trying to find from the in-person study?
% \end{itemize}

% }

% \hang{I don't feel the following contents are appropriate here}

% Reinforcement Learning (RL) is a powerful tool to be used in acquiring complex behaviors from high-dimensional specifications. 
% However, it is challenging to design a reward function that correctly encodes the task and allows the learning agent to be effectively optimized.
% Reward engineering creates a barrier between RL in the lab and RL in practice \cite{}.
% Inverse Reinforcement Learning (IRL) methods \cite{} enable learning a reward function directly from demonstrations, and demonstration is one of the most effective interaction archetypes \cite{koppol2021interaction}.
% IRL methods, on the other hand, are less preferred in many scenarios due to the learning efficiency \cite{}, or the requirements of using a  domain-specific regularizer. 
% Moreover, it is hard to learn a reliable reward function only using demonstrations due to the imperfections that wildly existed in human demonstrations.


% A promising direction is combining multiple teaching signals, including preference \cite{}, corrections \cite{}, and evaluations \cite{}. 
% The key insights of combining different teaching signals are: demonstrations are more informative but less accurate, while other teaching signals are more accurate but less informative. 
% This greatly increases the reliability of LfD methods and results in higher-quality reward functions.
% However,  
% giving preferences to two subtrajecotries is challenging, especially for non-experts. time to update their policy compared to virtual agents. 
% Moreover, asking for extra teaching signals, like correction, requires keeping humans in the loop for a long time since robots need more time to update their policy compared to virtual agents. 


% We, therefore, aim to learn accurate reward functions without keeping humans in the loop.
% We first 
% introduce a novel teaching signal called 
% \textit{progress} that annotates completion rates of tasks. 


% \section{Key idea}
% \hang{Put the key idea here as a reminder:
% The direction is to design an interactive Inverse Reinforcement Learning method for human to teach the robot while does not require humans to spend a long period time on the robot.

% Key idea: Using "progression" as extra constrains to learn the reward function and change the reward function to value function to reduce the learning efforts. 

% The constrains could be:
% \begin{itemize}
%     \item Preference/ranking (easiest). The subtrajectories with higher steepness should be more preferable than the subtrajectories with lower steepness.
%     \item Portions (middle). The portion of the rewards calculated by the  reward function should match the portion of the progression.
%     \item Rewards (hardest). The total rewards of a subtrajectory should match the total progression of a subtrajectory
% \end{itemize}

% Taking out the $a$ from the reward learning process should not significantly reduce the accuracy of the reward function, but would significantly reduce the learning cost. Moreover, the progression should just be about a state not state-action pairs (which might essentially be state-state transitions)






% Forgot Interactive GAIL. It is underdeveloped and one thing at a time!!!!


% implementation pipeline:
% \begin{enumerate}
%     \item get a demonstration recorder work.
%     \begin{enumerate}
%         \item get the orp working 
%         \item record object pos
%         \item record arm pos 
%         \item get the reference frame working
%         \item reply it with different initial position using the reference frame
%     \end{enumerate}
% \end{enumerate}

% }






% Applying machine learning technologies to robots had greatly increased robots' ability to learn new skills and accomplish complex tasks. 
% While machine learning methods require massive data, interactive learning methods enable robots to benefit from human teaching. 


% Human demonstrations are one of the most effective interactiion archetypes for humans to teach robots \cite.  
% Human teaching reduces the data needs and empowered the robot to adapt to human preferences. 
% humans could learn a skill by observing teachers, imitating teachers, and getting critics from teachers.  
% However, effectively learning from multiple types of teaching signals
% is difficult for robots. 




% Previous work [citations] tried to combine human demonstrations and preferences. 

% Reinforcement Learning (RL) is a powerful tool to be used in acquiring complex behaviors from high-dimensional specifications. 
% The reward functions used in RL, more often than not, are hand-coded by a human designer. 
% However, it is challenging to design a reward function that correctly encodes the task and allows the learning agent to be effectively optimized. 
% Reward engineering creates a barrier between RL in the lab and RL in practice.
% This challenge is further enlarged in Deep RL settings while Deep RL methods have achieved significant success in [citations].
% The reward function may not be able to be specified for tasks like making robots more socialized with humans [citation] or pre-designed reward functions may lead robots to behave unexpectedly such as autonomous vehicles learning to maintain high speed on the highway instead of driving down the road [cite]. 

% On the other hand, inverse reinforcement learning (IRL) methods enable learning a reward function directly from demonstrations. 
% However, there are many scenarios that IRL methods are less preferred. Methods that directly use demonstration, such as imitation learning [cite], have been shown generally more effective than IRL methods. IRL methods that use neural network usually requires domain-specific regularizer to 
% IRL methods trains over the whole trajectory.
% The learned reward function suffers from the imperfections of human demonstrations and high-quality demonstrations are rarely obtainable in the real world. 
% Although IRL methods have many limitations, the merits are promising. 
% The learned reward functions can be re-optimized when used in new environments [cite]. Inferring intentions from demonstrations rather than imitating enables the learning agent to be more robust to unfamiliar states [cite]. 

% The adversarial IRL methods [cite] demonstrated a promising direction for tackling difficult tasks by adaptively interacting with the environment. However, IRL methods assume that the learning agent could access high-quality or optimal demonstrations, which is hard to obtain even if the demonstrators are experts [cite]. In robotics, solving optimization problems in high-dimensional control space is more challenging[cite]. 

% Thus, IRL methods that only learn from demonstrations tend to learn suboptimal reward functions. 

% Prior work has succeeded by using human demonstrations to guide preference-based learning,  updating sub-trajectories of demonstrations via human preferences over sub-trajectories, \hang{need at least one more}.
% However,  these methods required keeping humans in the learning loop to provide teaching signals and asking humans to provide preferences over trajectories, which is hard for humans [cite].
% In this paper, we focus on learning accurate reward functions by integrating human demonstrations and human interactive teaching signals, while avoiding keeping humans in the loop during training.  
% The reward function is learned from demonstrations using adversarial learning, where the reward update process is constrained by [preference] (more preferable sub-trajectories should not receive less rewards than non-preferable sub-trajectories).


% \subsection{Progress}
% We define the \textit{progress} signal ranges from 0 to 100, representing the completion rate of a given task. A \textit{progress} value of 0 indicates that the task has not yet begun, while a value of 100 signifies task completion. 
% We aim to empower humans to better teach robots
% by incorporating \textit{progress} into the learning process.
% \hang{phrase this in a good form:
% We expect that a well-estimated \textit{progress} function is equal to a value function but requires fewer data to learn. Moreover, \textit{progress} can be used in many ways -- as evaluation (\textit{progress} increase as positive, decrease as negative), as preference(trajectories with a larger increase in \textit{progress} are more preferable), and as constraints in reward learning (the portion of rewards of a sub-trajectory should match its \textit{progress}).  
% }

% \textit{progress} can be used in many ways, such as evaluation (\textit{progress} increase as positive, decrease as negative), preference(trajectories with a larger increase in \textit{progress} are more preferable), and Inverse RL signal (for learning a \textit{progress} function)
% In this work, we use \textit{progress} as constraints to shape the learned reward function.  
% The key insights of using \textit{progress} are:
% \textit{progress} 
% to leverage their learning focus.

% by knowing the critical parts of a task performing, and knowing whether an action or a trajectory leads the robots toward the goal.



% \subsection{Matching \textit{progress} with A Reward Function}
% We hypothesized that a \textit{progress} function will be similar to a value function.  
% In the in-person study, we will use IRL methods to learn a reward function from each participant's demonstrations and thus get a value function using the learned reward function.
% In the online study, since the demonstrations are from an expert, we used pre-designed reward functions. 
% For the moving task, the reward is 85 (the average maximal reward of 20 participants) if the robot reaches the goal position. 
% For the pouring task, the reward for reaching the goal position is 40, and 60 for finishing the pouring. 
% For the spinning task, the reward is 10 for each step.

% We varied the reward decay factor $\gamma$ from 0.01 to 1 with a step of 0.01 to calculate the value function for each task. We found that none of the $\gamma$ creates a value function that fits the \textit{progress} well, which might indicate that human's expectation of the rewards from the future might be dynamic. Thus, we used a changing $\gamma$ that follows:
% \begin{equation}
%     \gamma = (current_step / all_steps ) / 30 + 0.67 
% \end{equation}
% .
% The results are shown in \autoref{fig:osr} (a), which shows that the value function with a dynamic $\gamma$  could fit the \textit{progress} function well. 


% \subsection{Change Points during the Task}
% Moreover, the ability to reflect the completion rate of the task

% \subsection{\textit{Progress} v.s. Accumulated Scalar Preference}


% \subsection{Workload}

% At the end of the online study, we presented participants with NASA TLX questionnaire to investigate if asking users to estimate the completion rate of the task based on the current state would require significantly more workload. 
% We compared the results on each dimension and the overall average. No statistical significance was found using paired-t tests (p > 0.1). 


% Previous work suggests that humans are not doing Inverse Reinforcement Learning (IRL)
% \hang{cite henny's paper} while they are learning from demonstrations or robot's behaviors.


% \section{Problem Statement}


% \section{Untangling Reward Function}
% One of the largest motivations that we want to use IRL is the learned reward function could be transferred to another scenario or used to train another robot. However, many IRL methods failed to recovery a robust reward functions due to learning from trajectory demonstrations.
% Ideally, the learn reward function should give rewards based on state-state transitions while the action could be arbitrary. 
% Learning from trajectory-based demonstrations leads the learned reward function to be shaped by dynamics of the system.

% \subsection{Reward shaping from system dynamics}
% The IRL problem can be interpreted as the solving the maximum likelihood problem. 
% \begin{equation}
%     maxlikelihood eq
% \end{equation}
% The optimal policy should remain unchanged, for any $\Phi: S \xrightarrow[]{} \mathbb{R}$, under the following reward transformation:
% \begin{equation}
%     rewar
% \end{equation}

% Assume the learned reward $r(s,a,s')$ is under a MDP $M$, and there is another MDP $M'$ that has different state transition probabilities. 
% The state transition functions are $T$ and $T'$ for MDP $M$ and MDP $M'$. 
% In this case, $T(s,a) \neq T'(s,a)$, which means that the $r(s,a,s')$ is not the same.
% This indicates that the reward functions recovered by IRL algorithms are actually shaped by the system dynamics. 


% \section{Effective Reward Learning}
% \hang{start with Interactive GAIL: i.e. using human feedback to constrain learned reward function 

% put the progression aside for a bit

% }

% Our goal is to precisely learn reward functions from few demonstrations.  
% It is hard to learn a high quality reward function from only using demonstrations \cite{} 
%  the imperfections are inevitably exist in human demonstrations
% %Moreover, the provided demonstration quality differs from user to user. 
% Even for experts, the quality of the sub-trajectories in one demonstration are not guaranteed to be consistent.
% On the other hand, humans perform better on evaluating than demonstrating, especially on robot assignments\hang{find citations if possible}, while the query efficiency of evaluations are relative lower than demonstrations. 
% Thus one core insight of our work is:
% \begin{enumerate}
%      \textit{The learning can be effectively performed by combing teaching signals that are less accurate but more informative with signals that are more accurate.}
% \end{enumerate}



% \hang{need rework}
% In this work, we proposed a new teaching signal \textit{progress}. 
% We claimed that progress captures the importance of the trajectories in a demonstration and progress is a human form of the reward function, which could benefit learning in multiple ways.

% We first conducted a two-phase online study with [NoP] participants and demonstrated that 
% progress conveys task statistics beyond critics and time, and inquiring progress does not necessitate higher cognitive loads compared to soliciting scalar feedback.
% Then we proposed an IRL algorithm as an instance of using progress to improve learning. 
% The method allows the robot to effectively learn reward functions from multiple persons without keeping humans in the loop.
% We validated our method with an open-space human study from non-expert users in a campus building. 

% % The online study is used to demonstrate that progress conveys information beyond critics including progress and mistakes, and is robust to tasks that do not have an end point. 
% % The in-person study further demonstrates that our IRL method learns an accurate reward function without keeping humans in the loop. 





% \subsection{Experimental Setup}
% We used a humanoid robot with a 7-degree of freedom Jaco2 arm for online study and a Kinova Gen 3 Lite arm for public space in-person study.
% We used a sugar-adding task for the online study and a candy-scooping task for the in-person study, shown in [Figure].
% For the sugar-adding task, the robot holds a cup, moves the cup to the target cup, pours the sugar into the target cup, and spins the stirrer in the target cup.   
% The online study has two phases. 
% In the first phase, we 
% break the task into three subtasks: reaching, pouring, and spinning, and only show them perfect demonstrations to reduce the workload from tasks and thus focus on the workload of giving different teaching signals. 
% In the second phase, we show participants four demonstrations, which are a perfect demonstration, a demonstration with imperfections, a demonstration with non-recoverable errors, and a demonstration with recoverable errors, to show the capability of progress. 

% For the candy scooping task, participants controlled the Gen3 Lite arm to scoop candies from a basket using a spoon and deliveries candies to a target zone. 




% \begin{enumerate}
%     \item \textbf{Task 1: reaching} In this task, the robot holds a cup and the goal is to move the cup to a desired location.  
%     \item \textbf{Task 2: pouring} The robot holds a cup with jelly balls, and the goal is to navigate to another cup and pours the jelly balls into it.
%     % \textbf{Task 2: scooping} In this task, the robot holds a spoon, and the goal is to scoop jelly balls from one cup to another. \hang{I prefer to change this task to a jelly ball pouring task, since it will be more consistent with task 1. 
%     \item \textbf{Task 3: spinning} In this task, the robot holds a spoon and spins the jelly balls in a pail. 
%     % \hang{\textbf{Task3: Capturing.}  }
    
% \end{enumerate}
% In the first task, the robot will lineally approach the task completion. 
% The second task has two sub-tasks, moving and pouring.
% The third task does not have a certain endpoint.
% The goal of the task design is to explore the performance of \textit{progress} in different tasks (simple task, segmentable task, and endless task). 
% \hang{q list: are three tasks strong enough? should I include failures? mistakes? what is the direction of writing: a new signal, and proves it works (demonstrate the advantages of progress)? or a new method with a new teaching signal (a new method to shape the reward function, works with preferences but better with progress)}


% \subsection{Online study procedure}
% \hang{edit corespondingly}
% We recruited two groups of 18 participants form AMT. 
% One group of participants was asked to give \textit{progress}, and the other group of participants was asked to give scalar evaluative feedback.
% Participants were redirected to our online study interface from the AMT platform after they clicked "Join".
% Participants gave scalar feedback or \textit{progress} to the robot behaviors by clicking a button with a corresponding value ({$0, 1, ..., 10$} for scalar feedback, \{$0\%, 10\%, ..., 100\%$\} for \textit{progress}).
% Each participant viewed three videos and each video is a recording of the robot performing one of the tasks.
% Before watching the videos and giving teaching signals,
% each task was briefly introduced to ensure that they had a consistent understanding of the task.
% The videos are from an expert's demonstrations, and participants gave a teaching signal after watching 10\% of the video. After participants finished giving teaching signals, a questionnaire was given. The questionnaire is NASA Task Load Index (TLX), which measures the total workload of giving \textit{progress} and preference. 

% \begin{figure*}[htbp]
%     \centering
%     \includegraphics[width = 1\textwidth]{online_study/online_study_1.png}
%     \caption{Online Study Results.}
%     \label{fig:online1}
% \end{figure*}
% \subsection{In-person Study procedure}
% \hang{more details for reproducibility}
% We recruited [XX] participants through email invitations, flyer distribution, and welcoming those who walked in to participate.
% The study was held in the lobby of a campus building.
% \hang{report gender, age, background}.
% Participants agreed to participate by signing a consent form.
% Then participants were introduced to the study.

% Participants' task was to control the arm using an Xbox controller to scoop the candies from a basket to a target zone.
% The spoon was already attached to the arm's gripper. 
% The basket's location was picked by participants, which could be any location in the workspace. 
% The study environment is shown in \autoref{}. 

% Participants had enough time to practice their skills.
% After practicing, they started to give demonstrations. 
% We videotaped their demonstrations using an overhead camera that only captured the workspace (i.e. participants were not shown in the video).
% We recorded the robot trajectories in 10 HZ.  
% For each participant, we only asked for one demonstration. 
% \hang{should we?}
% After getting one demonstration from a participant,
% we replayed their demonstration using the recorded robot trajectory.
% \hang{how should we replay the demo kinda depends on what learning algorithm we are going to use.}
% The replay might be slower compared to their demonstrations but followed the same time portion.  

% During the replay, the arm stopped 10 times. 
% Each time the arm stopped, the robot asked the participants 
% for both progress and scalar feedback.
% We did not ask participants to watch the replay twice and gave progress and scalar feedback separately since people would not be consistent with their teaching signals even with exactly the same behaviors \hang{cite steady paper here. however, asking for progress and preference together also will force them to associate preference with progress. }. 

% After collecting teaching signals, 
% we gave them a questionnaire about their experience of teaching the robot, and how they felt about two teaching signals. 
% Then, We claimed that progress captures the importance of the trajectories in a demonstration and progress is a human form of the reward function, which could benefit learning in multiple ways.
% the study ended and participants could take the candies with them. 

% \hang{draft of how we are going to use the data.}

% We used an Inverse RL method to learn from both human demonstrations, and preference or progress. 
% \hang{one problem with the current method is that current methods can not improve much from a few teaching signal. we at least should propose one tech in this paper. I have one, which is using teaching signals as constrains. Also, learning from demonstrations from multiple persons is hard. Not sure whether algs from prior work works}




% % Our in-person study shares the same tasks and the questionnaire as our online study to ensure the consistency of the results. The difference is that participants were asked to give demonstrations using Kinesthetic teaching instead of watching pre-recorded demonstrations from experts. 
% % We recruited participants from the campus area.
% % XX participants were recruited.
% % The arm was set to the gravity compensation model and could be moved by participants easily. 
% % Before giving the demonstration,
% % participants would be introduced to the task, and 
% % they had as much time as they wanted to practice.
% % Once participants were ready to give demonstrations, they could either inform the researcher by a doorbell or speech.
% % The robot arm and the cups would be randomly initiated in the task scenario. 
% % For each task, participants gave one demonstration. 
% % After participants demonstrated one task, 
% % we replayed their demonstration and asked them to give \textit{progress} for every 10\% steps. 
% % After finishing collecting demonstrations,
% % a questionnaire was given. 

% \subsection{Hypothesis}

% \begin{enumerate}

%     \item \textbf{H1.} \textit{progress} will increase as the robot is approaching task completion. 
%     \item \textbf{H2.} \textit{progress} will not be well-aligned with time. 
%     \item \textbf{H3.} \textit{progress} will not always be 100 even if the task was done. 
%     \item \textbf{H4.} \textit{progress} will be well associated with scalar feedback.
%     \item \textbf{H5.} Giving \textit{progress} will not add extra cognitive load to participants. 
% \end{enumerate}


% using a few demonstrations to extract an initial policy and further refining the extracted wih

% Combining human demonstrations and human feedback has multiple advantages. 

% \hang{ lfd requires a few demonstrations to learn a policy but lfhf requires thousands of labels, which is much more human effort. the policy learned from demonstrations only is less accurate since humans can not perfectly demonstrate, but human feedback can further shaped the learned policy and provide more accurate info }


% \hang{however, in prior work, demonstrations are from experts or pre-trained agents. They are either only contain one policy or not noisy enough even they injected noise. }
% \hang{progress, one policy, one corresponding evaluation.}


% An effective combination of human feedback and human demonstration should utilize the advantages of both signals and thus fulfill: 
% 1) demonstrations provide global guidance to improve sample efficiency for feedback 
% 2) feedback provides accurate local descriptions to mitigate the non-optimality of demonstrations
% 3) feedback provides insights to indicate trajectories with more preferred policies or critical behaviors. 


% However, feedback used in the combination is directly adapted from LfHF and only partially utilizes the advantages of combining with demonstrations. 
% The optimal form of feedback has not been fully considered. 

% The quality of a demonstration or a partial demonstration is typically assessed by comparing it to another\cite{palan2019learning, brown2019ranking, brown2020better}, which neglects the intrinsic quality of the demonstration itself and the fact that both demonstrations could be either good or bad.

% Our motivation is that human feedback should carry both objective and relative descriptions to better improve learning from human demonstrations, especially in cases where human demonstrations have multiple optimal policies or from non-experts.  

% an effective form of human feedback for human demonstrations should  and users should not be expected to provide high-quality demonstrations.  
% To this end, we (1) proposed a novel teaching signal that we assume that progress will better describe human demonstrations, especially their own demonstrations,  and (2) collected demonstrations and progress from non-experts and performed Weighted Behavior Cloning. 
% We published our collected demonstrations along with progress and human scalar evaluations.
% Our results indicated that progress contains information beyond good or bad, and also is capable of reflecting task completion. Using progress with demonstrations is more effective than using scalar evaluations. 

% In previous LfHF work, human demonstrations are used to boost the exploration process\cite{ibarz2018reward} or as annotations \cite{hester2018deep}
% of combining both human demonstrations and human feedback, preference\cite{ibarz2018reward, palan2019learning} and ranking\cite{brown2019ranking} are most commonly used.  

% However, most teaching signals prior work has used are either directly adapted from LfHF, which lessens the benefits of using human feedback and sometimes increases the human effort. 
 


% Meanwhile, preference learning and reinforcement learning methods are often used in IL, directly using signals has downsides, including keeping human in loop for long, feedback only has one side of information (local or global)

% We first demonstrated the capability of progress as a teaching signal. 
% We conducted a two-phase online study with 76 participants to collect progress with pre-recorded demonstrations from crowd users.
% We showed that progress could indicate: 1) if a partial trajectory is leading the robot towards or away from task completion; 2) the weight of a partial trajectory; 3) if the task is completed, while the workload is similar to providing scalar evaluation. 
% Then we conducted a public space study in a university building and collected non-expert demonstrations with progress over a pouring task. 
% All demonstrators we recruited were random people who walked by in a lobby of a university building. 
% After giving the demonstration, they were asked to provide ten progress and ten scalar evaluations. 
% We released all the demonstrations along with the progress and evaluations we collected. 
% We demonstrated that our method enables the robot to learn a better policy by using progress with a Weight Behavior Cloning algorithm. 

% We have three major contributions:
% \begin{enumerate}
%     \item Novel teaching signal: \textit{prgress}.
%     \item Non-expert demonstration data set. 
%     \item A new Weighted Behavior Cloning method. 
% \end{enumerate}
% \hang{revisit the last part once the in-person study in done or once we have the BC method}



% For instance, after providing demonstrations, users could further provide evaluations to the robot to shape its learned policies\cite{} or correct its wrong behaviors \cite{}.
% Inverse Reinforcement Learning (IRL) based on preference learning can also be used to deal with the imperfections in demonstrations. 

% \hang{
% 1. human feedback is powerful in improving learning but is not informative enough.
% Evaluations only describe good/bad of a partial trajectory. Preferences and rankings ignored the quality of a demonstration itself.  
% 2. A good teaching signal should reflect the quality of a partial trajectory itself, provide insights related to the whole trajectory, and relative importance compared to other partial trajectories.
% 3. We proposed progress. 
% 4. We demonstrated the capability of progress as feedback by comparing with scalar evaluation through a two-phase online study. We showed that progress can reflect weights, task completion, and good/bad indications without extra workload.

% for the following part, I have two ideas:
% one
% 5. We claimed progress would benefit learning not only in Interactive RL. It is effective if we combine it with demonstrations. We ran an open space study and collected demonstrations from non-experts with progress and preferences.
% 6. We demonstrated that progress outperforms preferences.

% two
% 5. We ran an in-person study by asking participants to teach the robot with progress and scalar evaluations. 
% 6. We demonstrated that progress is better than scalar evaluations even only part of information has been used. 

% }
% In recent years, we have witnessed a huge improvement in the capability of robots learning new skills or adapting to human preferences.   



% \begin{figure}
%     \centering
%     \includegraphics[width = 0.5\textwidth]{online_study/phase_2/delta_com.png}
%     \caption{Preference v.s rescaled delta progress. Similar but not worth to dig more.}
%     \label{fig:enter-label}
% \end{figure}



% \section{Learning alg}
% % \hang{using \textit{progress as constraints might not be the most effective way of using it }}
% % \hang{mention sth like directly learning a value function from \textit{progress} is doable but it requires a huge amount of human efforts}
% While performing a task, 
% it is natural for humans to subconsciously estimate the progress of a task.
% Common patterns are: estimating the progress linear (e.g. watching a movie) and estimating the progress segmented (e.g playing ball games). 
% To answer the questions that is \textit{progress} a reliable signal, would \textit{progress} work for a non-goal-based task, and what if some mistakes happened during the task performing,
% we performed an online study with two groups of participants.
% \subsection{Progress}
% Intuitively, the \textit{progress} of a task is similar to a value function, minor rewards on minor progress, large rewards on large progress, and only related to states instead of state-action-state transitions.

% Our goal is to precisely learn reward functions from a few demonstrations.  
% It is hard to learn a high-quality reward function from only using demonstrations \cite{} 
%  the imperfections inevitably exist in human demonstrations
% %Moreover, the provided demonstration quality differs from user to user. 
% Even for experts, the quality of the sub-trajectories in one demonstration is not guaranteed to be consistent.
% On the other hand, humans perform better on evaluating than demonstrating, especially on robot assignments\hang{find citations if possible}, while the query efficiency of evaluations is relatively lower than demonstrations. 
% Thus one core insight of our work is:
% \begin{enumerate}
%      \textit{The learning can be effectively performed by combing teaching signals that are less accurate but more informative with signals that are more accurate.}
% \end{enumerate}
% Due to the imperfections in human demonstrations, learning a stable model from only human demonstrations is challenging.  
% % Instead of viewing the inconsistency as flaws in human demonstrations, and trying to ignore it or reducing it, we believe it contains information for enabling more effective learning. \elaine{cite "Donut as I do" matt gombolay}

% % The gradients of the progression of sub-trajectories inside a demonstration  indicate the preference



% We decide to collect \textit{progress} only based on states rather than state-action pairs or trajectories, which means we will learn a value function through  \textit{progress} and use it to guide learning.

% The value function is:
% \begin{equation}
%     V^{\pi}(s) = \mathbb{E}_{a \sim  \pi} Q(s,a)
% \end{equation}

% \begin{equation}
%     \hat{r}(s,s') = V^\pi(s) -  V^\pi(s')
% \end{equation}


% The loss function is:
% \begin{equation*}
%    \text{IRL}_\psi(\pi_{E}))  = \arg \max_{c \in \mathbb{R}^{S \times A}} - \psi(c) + (\min_{\pi \in \Pi} -H(\pi) + \mathbb{E}[c(s,a)] )- \mathbb{E}_{\pi_E}[c(s,a)] +
%    \sum_{s_i,s_j \in s}^{} \frac{c(s_i,s_j)}{c(s)} - (pro(s_j) - pro(s_i))
% \end{equation*}


% \section{In-person Human study}
% We conducted an in-person study and collected both demonstrations and \textit{progress} from non-expert users. While the task is a goal-based task, we allowed participants to have preferences over the pouring speed to further validate the robustness of \textit{progress} and our learning algorithm.


% \subsection{Baselines}
% \begin{enumerate}
%     \item AIRL with two times of demonstrations
%     \item GAIL with two times of demonstrations
%     \item One SOTA preference + demonstration learning-based IRL method. 
% \end{enumerate}


% \section{Experiment}
% \hang{Do we need to compare the progress with preference? Since Preference is the most common signal used in IRL.}

% We conducted an open-space study to validate that our method enables effectively learning a reward function from multiple people without keeping humans in the loop. 
% We have [XX] participants provided demonstrations, progress, and feedback over a robot candy scooping task. 
% Participants were from a university building and the overall participation time was about 15 minutes. 
% The study was approved by the Institution of Reviewer Board. 



% \subsection{Open Space Study}


% \section*{Acknowledgments}

%% Use plainnat to work nicely with natbib. 


%\textbf{Inverse Reinforcement Learning}







% In online study phase two, we aim to demonstrate the robustness of progress with imperfect demonstration and compare the difference in information carried by preference and progress. 
% 

% Participants watched five demonstration replays: 
% \begin{enumerate}
%     \item A perfect demonstration. 
%     \item An imperfect demonstration but the task completion is not affected. 
%     \item A demonstration with recoverable mistakes and the mistakes have not been recovered.  
%     \item A demonstration with recoverable mistakes and the mistakes have been recovered. 
%     \item A demonstration with non-recoverable mistakes.  
% \end{enumerate}


% which are frequent in non-expert demonstrations. 
% \hang{I don't think this one is well supported, combining H3 and H4 would be good or change H4 to robust to }
% \noindent \textbf{H2.} Progress could indicate if the task is complete.

% \noindent \textbf{H3.} Progress allows the awareness of backtracking and unproductive explorations, which are non-optimal but not necessarily wrong. 


% Progress can detect ``undoing''/``backtracking'' and unproductive exploration/experimentation, which are common in non-expert demonstrations.} \elaine{something here about experimenting or backtracking not always bad}
% \hang{more like h5}





% \noindent \textbf{H5.} Delta progress (progress at the end minus progress at the start) indicates the importance of a partial trajectory related to the entire trajectory.






% \hang{intrinsic quality can say:
% progress has intrinsic information that is different from scalar feedback 
% scalar feedback describe the performance of the robot
% progress describe whether the robot is making progress
% one cares about quality
% one cares about whether the agent is acting towards finishing the task
% }
% \noindent \textbf{Indicating if the task is complete}
% \begin{itemize}

%     \item \textbf{Indicating if the task is complete}
%     \item \textbf{Indicating if the robot is acting towards finish the task}
%     \item \textbf{Indicating the importance of a partial demonstration}
%     \item \textbf{Robust to imperfections in demonstrations}
%     \item \textbf{No extra workload comparing to scalar evaluation}
% \end{itemize}

% \subsection{Phase One Results: the difference in workload is insignificant}




% \begin{figure}
%     \centering
%     \includegraphics[width = 0.5\textwidth]{in_person/Slide4.jpg}
%     \caption{Public Space Study}
%     \label{fig:enter-label}
% \end{figure}


% \begin{figure*}
%     \centering
%     \includegraphics[width = 1\textwidth]{Figures/Slide2.jpg}
%     \caption{Experiments}
%     \label{fig:experiment overview}
% \end{figure*}
